Polynomial approximations for the matrix logarithm with computation graphs

The most popular method for computing the matrix logarithm is a combination of the inverse scaling and squaring method in conjunction with a Pad\'e approximation, sometimes accompanied by the Schur decomposition. The main computational effort lies in matrix-matrix multiplications and left matrix division. In this work we illustrate that the number of such operations can be substantially reduced, by using a graph based representation of an efficient polynomial evaluation scheme. A technique to analyze the rounding error is proposed, and backward error analysis is adapted. We provide substantial simulations illustrating competitiveness both in terms of computation time and rounding errors.

==> Sec_comput_graphs.tex <==
% NO LONGER IN USE!

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational graphs for the matrix logarithm} \label{Sec_comput_graph}



%** Provide some table for reproducibility
%
%** $m_k$ is needed in the following section


==> Sec_error_testing.tex <==
\subsection{Rounding and approximation error experiments}


The three sets that have been employed in the numerical experiments are the same as those used in \cite{Iba2021Improved}. For conciseness, we omit the explanation of the sets and refer the reader to \cite[Section~3]{Iba2021Improved} for the description of  Set 1, Set 2 and Set 3.


%\begin{itemize}
%\item \textbf{Set 1}: one hundred diagonalizable $128\times 128$ complex matrices computed as $A=V \cdot D \cdot V^{T}$, where $D$ is a diagonal matrix with complex eigenvalues and $V$ is an orthogonal matrix such as $V=H/\sqrt{n}$, where $H$ is the Hadamard matrix of order $n$. The 2-norm of these matrices varies from $0.1$ to $300$. The \exact matrix logarithm was calculated as $\log{(A)}=V \cdot \log{(D)} \cdot V^{T}$.
%
%\item \textbf{Set 2}: one hundred non-dia\-go\-na\-li\-za\-ble $128\times128$ complex matrices computed as $A=V \cdot J \cdot V^{T}$, where $J$ is a Jordan matrix with complex eigenvalues whose algebraic multiplicity is randomly generated between $1$ and $3$. $V$, where  the first matrix $V$ is an orthogonal random matrix with elements in the interval $[-2.5, 2.5]$ and the elements the restant matrices are in the interval  $[-250,250]$. The 2-norm of these matrices range from $3.39$ to $337.72$. The \exact matrix logarithm was computed as $\log{(A)}=V \cdot \log{(J)} \cdot V^{T}$.
%
%\item \textbf{Set 3}: fifty-two matrices $A$ from the Matrix Computation Toolbox (MCT) \cite{higham2002test} and twenty from the Eigtool MATLAB Package (EMP) \cite{wright2009eigtool}, all of them with a $128\times128$ order. The \exact matrix logarithm has been calculated by using the MATLAB function \vpa from the Symbolic Math Toolbox with 256 decimal digits precision and the following method:
%
%\begin{enumerate}
%	\item
%	Use the MATLAB function \texttt{eig} for calculating a matrix $V$ and a diagonal matrix $D$ such that $A = V \cdot D \cdot V^{-1}$. If any of the elements of matrix $D$, i.e. the eigenvalues of matrix $A$, has a real value less than or equal to 0, it is replaced by the result of the sum of its absolute value and a random number in the interval $]0, 1[$. Thus, a new matrix $\widetilde{D}$ is generated. Next, matrices $\widetilde{A}$ and $L_1$ are calculated in the form $\widetilde{A} = V \cdot \widetilde{D} \cdot V^{-1}$ and $L_1= V \cdot \log(\widetilde{D}) \cdot V^{-1}$.
%	\item
%	Computing the matrix logarithm thanks to the \logm and \vpa functions, that is $L_2=\texttt{logm}(\widetilde{A})$. \logm is the built-in MATLAB function mention above \cite{al2012improved,al2013computing}.
%	\item
%	Considering the \exact  matrix logarithm of $\widetilde{A}$ only if \[\frac{{\left\| {{L_1} - {L_2}} \right\|}}{{\left\| {{L_1}} \right\|}} < u.\]
%\end{enumerate}
%
%Finally, for Test 3 a total of forty-six matrices were considered for the numerical experiments: forty from the MCT and six from the EMP. The others were excluded for the following reasons:
%\begin{itemize}
%	\item Matrices 17, 18 and 40 from the MCT and matrices 7, 9 and 14 from the EMP did not pass the previous procedure for the \exact matrix logarithm computation.
%	\item The relative error incurred by some of the codes in comparison was greater than or equal to unity for the matrices 4, 6, 12, 26, 35 and 38 belonging to the MCT and matrix 1, 4, 10, 19 and 20 pertaining to the EMP. The reason was the ill-conditioning of these matrices for the matrix logarithm function.
%	\item Matrices 2, 9 and 16, which are part of the MCT, and matrix 15 and 18, incorporated in the EMP, resulted in a failure because the function \sqrtmdbp, responsible for computing the principal square root of a matrix using the product form of the Denman-Beavers iteration,  did not converge after a maximum allowed number of 25 iterations.
%	\item Matrices 8, 11, 13 and 16 from the EMP were already incorporated in the MCT.
%\end{itemize}
%\end{itemize}
%

The relative error is computed as
$$
\textmd{Er(A)}=\frac{\| \log(A)-\widetilde{\log}(A)\|_2}{\left\Vert
	\log(A)\right\Vert_2},
$$
where $\log(A)$ is the \exact  solution and $\widetilde{\log}(A)$ denotes the matrix logarithm computed by the implementations in comparison. Tests were carried out on a Microsoft Windows 10 x64 PC computer with an Intel Core i7-6700HQ CPU @2.60Ghz processor and 16 GB of RAM, using MATLAB R2022b.


\begin{figure}[H]
	%\centering
	\begin{tabular}{cccccc}
		%\centering
		\includegraphics[width=6cm]{Figures/Test_1_normwise.eps}
		&\includegraphics[width=6cm]{Figures/Test_1_nprofile.eps}\\
		(\textbf{a}) Normwise relative errors. & (\textbf{b}) Performance profile.\\
		%\includegraphics[width=6cm]{Test_1_error_ratio.eps}
		%&\includegraphics[width=6cm]{Test_1_matrix_product_ratio.eps}\\
		%(\textbf{c}) Ratio of relative errors. & (\textbf{d}) Ratio of matrix products.\\
	\end{tabular}
	\caption{Experimental results for test set~1.}
	\label{fig_set1}
\end{figure}

Figures~\ref{fig_set1}a, \ref{fig_set2}a, and~\ref{fig_set3}a show the normwise relative errors of the three test sets. The solid line that appears is the products ${k_{\log}}u$, where ${k_{\log}}$ (or $cond$) represents the condition number of the matrix logarithm from the Matrix Function Toolbox~\cite{higham2002test}, and $u$ is the unit round off. The numerical stability of each method is evidenced if its errors are not much higher than this solid line. The matrices were ordered by decreasing value of $cond$. The  matrices 19, 21, 23, 27, 51 and 52 from the MCT and matrix 17 from the EMP were not plotted in Figure~\ref{fig_set3} because of the excessive condition number of the logarithm function, although these matrices were taken into account in the other graphs.


\begin{figure}[H]
	%\centering
	\begin{tabular}{cccccc}
		%\centering
		\includegraphics[width=6cm]{Figures/Test_2_normwise.eps}
		&\includegraphics[width=6cm]{Figures/Test_2_nprofile.eps}\\
		(\textbf{a}) Normwise relative errors. & (\textbf{b}) Performance profile.\\
		%\includegraphics[width=6cm]{Test_2_error_ratio.eps}
		%&\includegraphics[width=6cm]{Test_2_matrix_product_ratio.eps}\\
		%(\textbf{c}) Ratio of relative errors. & (\textbf{d}) Ratio of matrix products.\\
	\end{tabular}
	\caption{Experimental results for test set~2.}
	\label{fig_set2}
\end{figure}


According to these results, all codes are stable, especially the codes \logmpcg and \logmpol, whose relative errors were positioned in the lowest positions on the graphs. In most of the matrices, the functions \logmpcg and \logmpol, based on polynomial approximations, present smaller relative errors than the functions \logmnew,  \texttt{logm} and \texttt{logm\_ex} based on Pad\'e approximants.

Figures~\ref{fig_set1}b, \ref{fig_set2}b, and~\ref{fig_set3}b show the performance profile of the four codes where, on the $x$-axis, $\alpha$ took values from 1 to 5 with increments of 0.1. Given a specific value for the $\alpha$ coordinate, the parameter $p$ on the $y$-axis is the probability that the relative error of a particular algorithm is less than or equal to $\alpha$-times the smallest relative error over all the functions on the given test set. To reduce the influence of relative errors smaller than the unit roundoff in the performance profile pictures, these errors were modified according to the transformation described in \cite{DiHi13}.

The performance profiles confirm that \logmpcg and \logmpol based on polynomial approximations were the most accurate functions for the three matrix sets. In Tests 1 and 2, the performance graphs of both codes are similar, but in Test 3, code  \logmpol presents better performance, followed by code \logmpcg. However, Fig.~\ref{fig_set3}a shows that the the relative errors obtained by these two algorithms are of very similar order. The Pad\'e based codes \logmnew,  \texttt{logm} and \texttt{logm\_ex} had lower and very similar performance.


\begin{figure}[H]
	%\centering
	\begin{tabular}{cccccc}
		%\centering
		\includegraphics[width=6cm]{Figures/Test_3_normwise.eps}
		&\includegraphics[width=6cm]{Figures/Test_3_nprofile.eps}\\
		(\textbf{a}) Normwise relative errors. & (\textbf{b}) Performance profile.\\
		%\includegraphics[width=6cm]{Test_3_error_ratio.eps}
		%&\includegraphics[width=6cm]{Test_3_matrix_product_ratio.eps}\\
		%(\textbf{c}) Ratio of relative errors. & (\textbf{d}) Ratio of matrix products.\\
	\end{tabular}
	\caption{Experimental results for test set~3.}
	\label{fig_set3}
\end{figure}

